A novel shape matching descriptor for real-time hand gesture recognition

The current state-of-the-art hand gesture recognition methodologies heavily rely in the use of machine learning. However there are scenarios that machine learning cannot be applied successfully, for example in situations where data is scarce. This is the case when one-to-one matching is required between a query and a dataset of hand gestures where each gesture represents a unique class. In situations where learning algorithms cannot be trained, classic computer vision techniques such as feature extraction can be used to identify similarities between objects. Shape is one of the most important features that can be extracted from images, however the most accurate shape matching algorithms tend to be computationally inefficient for real-time applications. In this work we present a novel shape matching methodology for real-time hand gesture recognition. Extensive experiments were carried out comparing our method with other shape matching methods with respect to accuracy and computational complexity using our own collected hand gesture dataset and a modified version of the MPEG-7 dataset.%that is widely used for comparing 2D shape matching algorithms. Our method outperforms the other methods and provides a good combination of accuracy and computational efficiency for real-time applications.

==> fig/hist/distributions.tex <==
\begin{tabular}{cc}
\small
\centering
\setlength\tabcolsep{0pt}

\extfig{art-20}
{
\begin{tikzpicture}
\begin{axis}[
	width=.55\linewidth,
	height=.38\linewidth,
	font=\small,
	ybar,
	xmin=0,
	xmax=1.5,
	ymin=0,
	xlabel={average loss},
	ylabel={\# examples},
	yticklabels={,,},
	xtick style={draw=none},
	ytick style={draw=none},
	% xtick pos=bottom,
	% ytick pos=left,
	grid=none,
	bar/.style={thin,fill opacity=0.5,bar width=0.029497127532958984},
]
\addplot[red, fill=red, bar] table[x=bins,y=bad] \weightHistInit; \leg{correct}
\addplot[blue,fill=blue,bar] table[x=bins,y=ok]  \weightHistInit; \leg{incorrect}
\addplot[domain=0.2:1.5,smooth,red] table[x=x_noisy,y=kde_noisy] \labelkdea;
\addplot[domain=0:0.5,smooth,blue] table[x=x_clean,y=kde_clean] \labelkdea;
\end{axis}
\end{tikzpicture}
}

&

\extfig{art-40}
{
\begin{tikzpicture}
\begin{axis}[
    width=.55\linewidth,
    height=.38\linewidth,
    font=\small,
    ybar,
    xmax=3.5,
    xmin=0,
    ymin=0,
    xlabel={average loss},
    yticklabels={,,},
    xtick style={draw=none},
    ytick style={draw=none},
    % xtick pos=bottom,
    % ytick pos=left,
    grid=none,
    bar/.style={thin,fill opacity=0.5,bar width=0.062066144943237304},
]
\addplot[red, fill=red, bar] table[x=bins,y=bad] \weightHistMiddle;
\addplot[blue,fill=blue,bar] table[x=bins,y=ok]  \weightHistMiddle;
\addplot[domain=0:4,smooth,red] table[x=x_noisy,y=kde_noisy] \labelkdeb;
\addplot[domain=0:3,samples=200,smooth,blue] table[x=x_clean,y=kde_clean] \labelkdeb;

\end{axis}
\end{tikzpicture}
}

\\
(a) 20\% uniform &
(b) 40\% uniform \\

\extfig{query-1}
{
\begin{tikzpicture}
\begin{axis}[
	width=.55\linewidth,
	height=.38\linewidth,
	font=\small,
	ybar,
	xmin=0,
	xmax=1.5,
	ymin=0,
	xlabel={average loss},
	ylabel={\# examples},
	yticklabels={,,},
	xtick style={draw=none},
	ytick style={draw=none},
	% xtick pos=bottom,
	% ytick pos=left,
	grid=none,
	bar/.style={thin,fill opacity=0.5,bar width=0.02777163028717041},
]
\addplot[red, fill=red, bar] table[x=bins,y=bad] \labelquerya; %\leg{correct}
\addplot[blue,fill=blue,bar] table[x=bins,y=ok]  \labelquerya; %\leg{incorrect}
\addplot[domain=0.2:1.5,smooth,red] table[x=x_noisy,y=kde_noisy] \labelqueryakde;
\addplot[domain=0:0.5,smooth,blue] table[x=x_clean,y=kde_clean] \labelqueryakde;
\end{axis}
\end{tikzpicture}
}

&

\extfig{query-2}
{
\begin{tikzpicture}
\begin{axis}[
    width=.55\linewidth,
    height=.38\linewidth,
    font=\small,
    ybar,
    xmax=1.5,
    xmin=0,
    ymin=0,
    xlabel={average loss},
    yticklabels={,,},
    xtick style={draw=none},
    ytick style={draw=none},
    % xtick pos=bottom,
    % ytick pos=left,
    grid=none,
    bar/.style={thin,fill opacity=0.5,bar width=0.02024201154708862},
]
\addplot[red,fill=red,bar] table[x=bins,y=bad]  \labelqueryc;
\addplot[blue,fill=blue,bar] table[x=bins,y=ok]  \labelqueryc;
\addplot[domain=0:4,smooth,red] table[x=x_noisy,y=kde_noisy] \labelqueryckde;
\addplot[domain=0:3,samples=200,smooth,blue] table[x=x_clean,y=kde_clean] \labelqueryckde;

\end{axis}
\end{tikzpicture}
}

\\
(c) task 1 &
(d) task 2

\end{tabular}


==> fig/hist/histbal.tex <==
\begin{tabular}{cc}
\small
\centering
\setlength\tabcolsep{0pt}

\extfig{histograms-before}
{
\begin{tikzpicture}
\begin{axis}[
	width=2\linewidth,
	height=0.5\linewidth,
	font=\small,
	ybar,
	xmin=-1,
	xmax=75,
	ymin=0,
	ymax = 1.5,
	%xlabel={query ID},
	ylabel={correct},
	yticklabels={,,},
	xtick style={draw=none},
	ytick style={draw=none},
	% xtick pos=bottom,
	% ytick pos=left,
	grid=none,
		bar/.style={thin,fill opacity=0.5,bar width=1},
]
\addplot[red, fill=red, bar] table[x=x,y=before] \labelhistograms; \leg{before}
%\addplot[blue,fill=blue,bar] table[x=x,y=uniform]  \labelhistograms; \leg{uniform}
%\addplot[green,fill=green,bar] table[x=x,y=entropy]  \labelhistograms; \leg{entropy}
\end{axis}
\end{tikzpicture}
}
& 
\\
\extfig{histograms-uniform}
{
\begin{tikzpicture}
\begin{axis}[
	width=2\linewidth,
	height=0.5\linewidth,
	font=\small,
	ybar,
	xmin=-1,
	xmax=75,
	ymin=0,
	ymax = 1.5,
	%xlabel={query ID},
	ylabel={correct},
	yticklabels={,,},
	xtick style={draw=none},
	ytick style={draw=none},
	% xtick pos=bottom,
		% ytick pos=left,
	grid=none,
	bar/.style={thin,fill opacity=0.5,bar width=1},
]
%\addplot[red, fill=red, bar] table[x=x,y=before] \labelhistograms; \leg{before}
\addplot[blue,fill=blue,bar] table[x=x,y=uniform]  \labelhistograms; \leg{uniform}
%\addplot[green,fill=green,bar] table[x=x,y=entropy]  \labelhistograms; \leg{entropy}


\end{axis}
\end{tikzpicture}
}
&
\\

\extfig{hist-entropy}
{
\begin{tikzpicture}
\begin{axis}[
	width=2\linewidth,
	height=0.5\linewidth,
	font=\small,
	ybar,
	xmin=-1,
	xmax=75,
	ymin=0,
	ymax = 1.5,
	xlabel={query ID},
	ylabel={correct},
	yticklabels={,,},
	xtick style={draw=none},
	% xtick pos=bottom,
	% ytick pos=left,
	grid=none,
	bar/.style={thin,fill opacity=0.5,bar width=1},
]
%\addplot[red, fill=red, bar] table[x=x,y=before] \labelhistograms; \leg{before}
%\addplot[blue,fill=blue,bar] table[x=x,y=uniform]  \labelhistograms; \leg{uniform}
\addplot[green,fill=green,bar] table[x=x,y=entropy]  \labelhistograms; \leg{entropy}


\end{axis}
\end{tikzpicture}
}
\end{tabular}

==> tex/plots-none.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/plots.tex <==
%------------------------------------------------------------------------------
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,shapes,calc,matrix,fit,positioning,backgrounds,decorations.markings}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.9}
\usepackage{xstring}

%------------------------------------------------------------------------------

\usepgfplotslibrary{external}
\tikzexternalize[prefix=fig/extern/]
\newcommand{\extfig}[2]{\tikzsetnextfilename{#1}{#2}}
\newcommand{\noextfig}[1]{\tikzset{external/export next={false}}{#1}}
\newcommand{\extdata}[1]{\input{#1}}
\IfBeginWith*{\jobname}{fig/extern/}{\finalcopy}{}

%-----------------------------------------------------------------------------
% tikz styles

\tikzstyle{every picture}+=[
	remember picture,
	every text node part/.style={align=center},
	every matrix/.append style={ampersand replacement=\&},
]
\tikzstyle{tight} = [inner sep=0pt,outer sep=0pt]
\tikzstyle{node}  = [draw,circle,tight,minimum size=12pt,anchor=center]
\tikzstyle{op}    = [draw,circle,tight]
\tikzstyle{dot}   = [fill,draw,circle,inner sep=1pt,outer sep=0]
\tikzstyle{pt}    = [fill,draw,circle,inner sep=1.5pt,outer sep=.2pt]
\tikzstyle{box}   = [draw,thick,rectangle,inner sep=3pt]
\tikzstyle{high}  = [black!60]
\tikzstyle{group} = [high,box,opacity=.5]
\tikzstyle{rectc} = [tight,transform shape]
\tikzstyle{rect}  = [rectc,anchor=south west]

%-----------------------------------------------------------------------------
% framed figures

\newcommand{\framed}[3][1]{\extfig{#2}{\tikz{
	\node[tight](a){\fig[#1]{#3}};
	\node[tight,draw=gray,fit=(a)]{};
}}}

%-----------------------------------------------------------------------------

\newcommand{\leg}[1]{\addlegendentry{#1}}

\tikzset{every mark/.append style={solid}}
\pgfplotsset{%smooth,
	grid=both, width=\columnwidth, try min ticks=5,
	every axis/.append style={font=\small},
	every axis plot/.append style={thick,mark=none,mark size=1.8,tension=0.18},
	legend cell align=left, legend style={fill opacity=0.8},
	xticklabel={\pgfmathprintnumber[assume math mode=true]{\tick}},
	yticklabel={\pgfmathprintnumber[assume math mode=true]{\tick}},
	nodes near coords math/.style={
		nodes near coords={\pgfmathprintnumber[assume math mode=true]{\pgfplotspointmeta}},
	},
}

\pgfplotsset{
	dash/.style={mark=o,dashed,opacity=0.6},
	dott/.style={mark=o,dotted,opacity=0.6},
	nolim/.style={enlargelimits=false},
	plain/.style={every axis plot/.append style={},nolim,grid=none},
}
\newcommand{\kilo}[1]{\thisrow{#1}/1000}


